Learning to Coordinate for a Worker-Station Multi-robot System in Planar Coverage Tasks

For massive large-scale tasks, a multi-robot system (MRS) can effectively improve efficiency by utilizing each robot's different capabilities, mobility, and functionality. In this paper, we focus on the multi-robot coverage path planning (mCPP) problem in large-scale planar areas with random dynamic interferers in the environment, where the robots have limited resources. We introduce a worker-station MRS consisting of multiple workers with limited resources for actual work, and one station with enough resources for resource replenishment. We aim to solve the mCPP problem for the worker-station MRS by formulating it as a fully cooperative multi-agent reinforcement learning problem. Then we propose an end-to-end decentralized online planning method, which simultaneously solves coverage planning for workers and rendezvous planning for station. Our method manages to reduce the influence of random dynamic interferers on planning, while the robots can avoid collisions with them. We conduct simulation and real robot experiments, and the comparison results show that our method has competitive performance in solving the mCPP problem for worker-station MRS in metric of task finish time.

==> p_env_modeling.tex <==
\newcommand{\reward}[1]{(^{#1} r)_t^i}

\section{Environment Modeling}\label{sec:env_modeling}
In order to solve the planning problem formulated in Eq.~\ref{eq:obj_func} using Deep Reinforcement Learning (DRL) based approaches, we first elaborate how the environment is modeled, including the coverage task, the observation space, action space as well as the reward design.

